Second-Order Perturbation Theory-Based Digital Predistortion for Fiber Nonlinearity Compensation

The first-order (FO) perturbation theory-based nonlinearity compensation (PB-NLC) technique has been widely investigated to combat the detrimental effects of the intra-channel Kerr nonlinearity in polarization-multiplexed (Pol-Mux) optical fiber communication systems. However, the NLC performance of the FO-PB-NLC technique is significantly limited in highly nonlinear regimes of the Pol-Mux long-haul optical transmission systems. In this paper, we extend the FO theory to second-order (SO) to improve the NLC performance. This technique is referred to as the SO-PB-NLC. A detailed theoretical analysis is performed to derive the SO perturbative field for a Pol-Mux optical transmission system. Following that, we investigate a few simplifying assumptions to reduce the implementation complexity of the SO-PB-NLC technique. The numerical simulations for a single-channel system show that the SO-PB-NLC technique provides an improved bit-error-rate performance and increases the transmission reach, in comparison with the FO-PB-NLC technique. The complexity analysis demonstrates that the proposed SO-PB-NLC technique has a reduced computational complexity when compared to the digital back-propagation with one step per span.

==> maplestd2e.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% <PRE>
\def\MapleNameDef $#1: #2.#3${\expandafter\gdef\csname Maple@#1\endcsname{#2}}
\def\MapleInfoDef $#1: #2 #3${\expandafter\gdef\csname Maple@#1\endcsname{#2}}
\MapleNameDef $RCSfile: maple2e.sty,v $
\MapleInfoDef $Revision: 1.16 $
\MapleInfoDef $Date: 2005/03/17 15:58:14 $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Package: \Maple@RCSfile\space \Maple@Date\space v\Maple@Revision}
\ProvidesPackage{maplestd2e}[\Maple@Date\space\Maple@RCSfile
Maple Latex Style Package -- \Maple@Date\space\Maple@RCSfile]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Copyright (c) 1994--2005 by Waterloo Maple Inc., all rights reserved.
%
% Permission is granted to use this package without charge. It may
% be redistributed providing that it is distributed as is
% and without charge.  You may modify these macros for your own use,
% and redistribute them, subject to the following conditions.
%
% 1. The package name used for any modified version of this file is 
%    different from maple2e and the file name used is different from
%    maple2e.sty
%
% 2. You acknowledge this copyright notice and this file as the source.
%
% 3. The new file is redistributed under the same terms and conditions 
%    as indicated here, including a version of this notice modified to
%    refer to the new file and/or package name.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
% Package:  maple2e 
%
% This package defines the latex macros used by "Export to LaTeX" 
% It makes use of several sub-packages.
% 
% mapleenv - Maple Environments used to mark mapleinput, mapleoutput,
% mapletab - Maple Macros to display tables (spreadsheets)
% mapleplots - Maple macros to display plots.
%
% See the comments in maplenv.sty for a more detailed discussion of
% the special environments such as
%
%	\begin{mapleinput} ... \end{mapleinput}
%	\begin{maplelatex} ... \end{maplelatex}
%
% and for details about macros such as
%
%	\mapleinline <status> <type> <verbatim code> <latex code>
%	\maplemultiline{ ... }
%
% which are used to control style and to embed raw Maple data.
% 
% USAGE:
%
%	To use this package, add the line  
%
%	\usepackage{maple2e} to 
%
%	your document preamble.  If you are using a specific plot
%	driver such as dvipsone, then add its name as an option as
%	in:
%
%	\usepackage[dvipsone]{maple2e}
%
%	The default option value is "dvips".
%
%	If you wish to preview your document, ignoring plots, use
%	the "noplots" option.
%
%	The only options available are precisely those needed to
%	control plotting.  Plots are handled by the standard LaTeX2e
%	graphics package and for LaTeX are restricted to postscript.
%	 
% NOTES:
%
%	It is an easy extension of this code to other plot file formats.
%	All that is needed is a new definition of \mapleplot
%	to invoke the graphics code of your choice.
%
%	To adjust the spacing around the Maple environemnts, edit
% 	change the entries in the file mapleenv.def
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Package Options
%
\newif\ifnoplots\noplotsfalse
\DeclareOption{noplots}{
    % \PassOptionsToPackage{dvips}{epsfig}
    \noplotstrue
}
\DeclareOption{dvips}{
    % \PassOptionsToPackage{dvips}{epsfig}
    \edef\Driver{dvips}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvips driver}
      \usepackage[dvips]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvi2ps}{
    \edef\Driver{dvi2ps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvips driver}
      \usepackage[dvi2ps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvilaser}{
    \edef\Driver{dvilaser}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvilaser driver}
      \usepackage[dvilaser]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvipsone}{
    \edef\Driver{dvipsone}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvipsone driver}
      \usepackage[dvipsone]{epsfig}
      %%% \let\mapleplot\mapleplotname %%%
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvitops}{
    \edef\Driver{dvitops}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvitops driver}
      \usepackage[dvitops]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dviwindo}{
    \edef\Driver{dviwindo}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dviwindo driver}
      \usepackage[dviwindo]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{emtex}{
    \edef\Driver{emtex}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for emtex driver}
      \usepackage[emtex]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{pubps}{
    \edef\Driver{pubps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for pubps driver}
      \usepackage[pubps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{textures}{
    \edef\Driver{textures}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for textures driver}
      \usepackage[textures]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{xdvi}{
    \edef\Driver{xdvi}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for xdvi driver}
      \usepackage[xdvi]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dvitps}{
    \edef\Driver{dvitps}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dvitps driver}
      \usepackage[dvitps]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{dviwin}{
    \edef\Driver{dviwin}
    \AtEndOfPackage{
      \typeout{ ...configuring graphics for dviwin driver}
      \usepackage[dviwin]{epsfig}
      \let\mapleplot\epsfigmapleplot
      \let\imapleplot\mapleplot
    }
}
\DeclareOption{oztex}{
    \edef\Driver{oztex}
    \AtEndOfPackage{
      \typeout{ ...Configuring graphics for OzTex, rotation not supported}
      \usepackage[oztex]{epsfig}
      \let\mapleplot\oztexmapleplot
      \let\imapleplot\mapleplot
    }%
}
\DeclareOption{SWP}{
    \edef\Driver{SWP}
    \AtEndOfPackage{
      \typeout{ ...Configuring graphics for Scientific Work Place}
      \let\mapleplot\swpmapleplot
      \let\imapleplot\mapleplot
    }
}
% \ExecuteOptions{dvips}  % default's to dvips driver
\ProcessOptions*
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Utilities and Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Miscelaneous utilities used to define the main Maple environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Maple Utility Macros}
%
% Utilities for changing character codes
%
\def\MakeTab#1{\catcode `#1 = 4 }      		% &
\def\MakeParameter#1{\catcode `#1 = 6 }		% #
\def\MakeSuperScript#1{\catcode `#1 = 7 }	% ^
\def\MakeSubScript#1{\catcode `#1 = 8 }		% _
\def\MakeLetter#1{\catcode `#1 = 11 }
\def\MakeOther#1{\catcode`#1 = 12 }
\def\MakeActive#1{\catcode `#1 = \active\relax }
\def\MakeTabActive{\MakeActive{\^^I}}
\def\MakeEolActive{\MakeActive{\^^M}}
%
\@ifundefined{dospecials}{%
\gdef\dospecials{\do\ \do\\\do\{\do\}\do\$\do\&\do\#\do\^\do\_\do\%\do\~}%
}{\relax}%
\@ifundefined{postdospecials}{%
\gdef\postdospecials{%
\catcode`\\\z@%
\catcode`\{\@ne%
\catcode`\}\tw@%
\catcode`\ 10%
\catcode`\&11}%
}{\relax}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% In a Maple tty environment every line is treated as a paragraph.
% The behavior at the end of every Maple paragraph (line) is given
% by, thereby inhibiting page breaks in such environments.
\def\@MaplePar{\nopagebreak[3]\par\@@par}%
% \def\@MaplePar{\nopagebreak[3]\EveryParZ\@@par}%
%
\newif\if@IgnoreNewLine
\@IgnoreNewLinetrue
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Characters requiring special treatment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-- Spaces
\def\MapleSpace{\ }
\def\@ObeySpaces{\MakeActive{\ }\@@ObeySpaces\relax}
{\MakeActive{\ }\gdef\@@ObeySpaces{\edef {\MapleSpace}}}

%-- BackSlashes

{\catcode`| = 0 |catcode`\\ = 12 |gdef|BackSlash{\}}

%-- Tabs

\newdimen\@MapleTabSize
\def\@ObeyTabs{\MakeTabActive\@@ObeyTabs\relax}
{\MakeTabActive\gdef\@@ObeyTabs{\def^^I{\@MapleTab}}}
\def\@MapleTab{%
  \leavevmode   % ensure that we are in horizontal mode
  \egroup      % Terminate box register 0
  \dimen0=\wd0 % store its length and round up to next stop
  \divide\dimen0 by \@MapleTabSize
  \advance\dimen0 by 1sp
  \multiply \dimen0 by \@MapleTabSize
  \wd0 = \dimen0
  \box0
  \setbox0 = \hbox\bgroup
}

%-- End of Line Character

\def\@ObeyEol{\MakeEolActive\@@ObeyEol\relax}%
{\MakeEolActive\gdef\@@ObeyEol{\let^^M=\@MapleEol}}
\def\@MapleEol{%
  \if@IgnoreNewLine
  \else
    \leavevmode%
    \egroup%
    \box 0%
    \@MaplePar%
  \fi
  \@IgnoreNewLinefalse
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definitions of Utilities for the Main Maple Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These Macros are the common elements of the verbatim like environents.
% The spacing above and below the environment should is done in the 
% environment preamble instead of here to enable this to be used in a 
% variety of such environments.

% \newtoks\MapleIOType \MapleIOType = {a}
\edef\@MapleQuiet{q}      % indicates a silent command or result
\edef\@MapleVerbose{a}    % The standard behavior in which
                          % results are generated and displayed.
\edef\@MapleNoPrompt{np}  % specify no prompts in environment
\edef\@MaplePrompt{p}     % specify prompts for this environment
\edef\@MapleNoInput{ni}   % No input appears in output stream.
\edef\@MapleNoOutput{no}  % No output appears in outputstream.

% The next macro is used by the verbatim like environments to
% reset character codes, and change the treatment of new lines, etc.
% Actions  can be made conditional on the value of \@MapleIOType which
% is always set to 'a' , or to 'q' as in the value of the 
% optional parameter used in \begin{mapleinput}[q]

\newtoks\MapleListCorrection  \MapleListCorrection={}
\def\@SetupMapleTty#1{%
\par\@endpefalse   %% to clear the \@endpetrue done in \mapleinput
\begingroup  %% this is the real start of the special environment. 
  %%%  Compute and set tab positions
  \setbox 0 = \hbox{\@MapleFont X}
  \@MapleTabSize = \wd0
  \multiply\@MapleTabSize by \MapleTab
  \setbox0 = \hbox{\relax}  % Clearing \box 0
  %%% paragraph dimensions and line spacing
  \rightskip = 0pt 
  \parindent = 0pt
  \parskip = 0pt 
  \ifnum\@listdepth>0%
        \MapleListCorrection={\hskip-\@totalleftmargin\relax }
        \LeftMapleSkip= 0em 
  \else
        \MapleListCorrection={\hskip 0ex\relax }
  \fi
  \setlength{\leftskip}{\LeftMapleSkip}
  \addtolength{\leftskip}{\@totalleftmargin}
  \parfillskip = 0pt plus 1fil
  %
  %%%  The next two parameters may have been changed 
  %%%  by a \raggedright so they are reset here.
  \spaceskip = 0pt   \xspaceskip = 0pt
  %
  %%%  Set this flag to 0 if the \begin{...} is to appear on a
  %%%  separate line of the source file.
  \ifnum #1 = 0 \@IgnoreNewLinetrue\else\@IgnoreNewLinefalse\fi%
  %
  %%% Describe how to handle every paragraph (recall paragraph == line )
  %% \@MapleFont%
  \everypar = {\EveryParZ}%
  \def\EveryParZ{%
    \ifMaplePrompt
    \the\MapleListCorrection
    \the\MaplePromptString
    \MaplePromptString = \MaplePromptSecondary
    \MapleListCorrection = {\hskip 0pt\relax}
    \fi
    \setbox0 = \hbox \bgroup
  }%
%
%%%  Choose the type size and font -  The order of these commands
%%%  may be important.
\@MapleFont%
\lineskiplimit=0\normalbaselineskip%
\baselineskip=0.85\normalbaselineskip%
\@noligs%
\let\do\@makeother\dospecials%
\catcode ``=\active%
\frenchspacing%
\@ObeySpaces% 
\@ObeyTabs%
\@ObeyEol%
}

% Exit the special tty environments
\def\@EndMapleTty{%
\endgroup%% matches the \begingroup inside of @SetupMapleTty
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The following Macros start the various Verbatim like environments
% for special Maple regions.  These calls set up the 
% scanning for the environment terminator.
%
% A conditional parameter as in \begin{...}[q] etc. denotes a
% special class of Maple Regions.

\begingroup
  \catcode`| = 0  % becomes the escape character
  \catcode`( = 1  % becomes a begin group
  \catcode`) = 2  % becomes an end group
  \catcode`@ = 11 % becomes a regular character (for macro names)
  \catcode`\{ = 12 % becomes an other character
  \catcode`\} = 12 % becomes a other character
  \catcode`\\ = 12 % becomes a other character
%
%  type a   standard (verbose) usage
%  type q   quiet command
%  type np  no prompt  (imapleinput only at this time...)
%  type ni  no input  
%  type no  no output  
%
% -- Maple Inert Input  
|gdef|@BeginIMapleInput#1\end{imapleinput}(%
|MaplePrompttrue%
#1%
|end(imapleinput))%
%
% -- Inert TTY Output
|gdef|@BeginIMapleTtyout#1\end{imaplettyout}(%
|vskip|AboveMapleSkip%  extra vspace is needed here
|MaplePromptfalse
#1%
|end(imaplettyout))%
%
% -- Fixed Width
|gdef|@BeginMapleFixedWidth#1\end{MapleFixedWidth}(%
|vskip|AboveMapleSkip%  extra vspace is needed here
|MaplePromptfalse
#1%
|end(MapleFixedWidth))%
% -- TTY Input 
|gdef|@BeginMapleInput[#1]#2\end{mapleinput}(%
|edef|@MapleIOType(#1)%
|gdef|MapleIOType(#1)%
|ifx|@MapleIOType|@MapleNoPrompt|MaplePromptfalse|fi%
|ifx|@MapleIOType|@MapleNoInput|edef|@MapleIOType(q)|fi%
|ifx|@MapleIOType|@MapleQuiet%
|typeout(.............Quiet Maple Command #1)%
|removelastskip%
|else%
%|typeout(.............Verbose Maple Command)%
#2%
|fi%
|end(mapleinput))%
%
% -- TTY Output
|gdef|@BeginMapleTtyout[#1]#2\end{maplettyout}(%
%%|typeout(TTYout Environment of type #1)%
|edef|@MapleIOType(#1)%
|gdef|MapleIOType(#1)%
|ifx|@MapleIOType|@MaplePrompt|MaplePromptfalse|fi%
|ifx|@MapleIOType|@MapleNoOutput|edef|@MapleIOType(q)|fi%
|ifx|@MapleIOType|@MapleQuiet%
|typeout(.............Quiet Maple Tty Out)%
|else%
#2%
|fi%
|end(maplettyout))%
%
% -- Suppressed Latex Output
|gdef|@GobbleMapleLatex#1\end{maplelatex}(%
|end(maplelatex))%
|endgroup
%
\@ifundefined{]}{\gdef\[{$}}{\relax}
\@ifundefined{[}{\gdef\]{$}}{\relax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Standard Maple Environments
%
% Environments for Export to LaTeX
%
% This package defines the environments used by Maple's
% "Export to Latex" facility.  In addition, each of the environments 
% accepts an optional parameter.  For example, for example,
% Maple Input lines accept any of:
%
%      \begin{mapleinput}...\end{mapleinput},   (default)
%
% The contents of such an environment are in terms of mapleinline.
%
% The "Export to LaTeX" facility of the Maple worksheet does not use any
% of the optional parameters.  They exist to provide the additional
% control needed for reprocessing long LaTeX manuscripts and which is
% carried out by a special "Maple Filter".
% 
% Maple output can occur in several forms.  Maple's "prettyprint" output,
% as well as error messages and warnings, is encapsulated as
%
% 	        \begin{maplettyout}...\end{maplettyout} 
%
% "Export to Latex" generates LaTeX code for the entire worksheet. 
%  The displayed mathematics output is controlled to fit a
%  user specified line width and appears inside the environment
%
% 	\begin{maplelatex}...\end{maplelatex}
%
% Maple generated plots are exported as postscript files.
% The resulting files are included in the LaTeX document 
% by using the macro call
%
%  	\mapleplot{filename}
%
% On processing by LaTeX, the postscript code from the 
% indicated file is read into "dvi" file and a display is 
% generated at that point in the document.  The plot dimensions 
% are specified as \MaplePlotHeight and \MaplePlotWidth.
%
% The actual embedding is accomplished using the LaTeX2e graphics 
% package.  This style file has been tested with the following dvi to 
% PostScript conversion programs:
%
%     dvips 
%     dvipsone
%
% ----------------------------------------------
% Environments that ignored by the Maple Filter
% ----------------------------------------------
% The Maple Filter is a special version of Maple that can read
% and update latex files which have been developed using these
% macros.  There is a need, in such tex files, to display information
% in the same manner as the preceding manner and yet guarantee that
% the information is not changed by the Maple Filter.
% The macros are identical to those describe above, but with each 
% name preceded by an "i".
%
%   \begin{imapleinput}...\end{imapleinput}  like mapleinput
%   \begin{mapleinput}[p]...\end{imapleinput} as above, default case
%   \begin{imaplelatex}...\end{imaplelatex} like maplelatex
%   \imapleplot{filename}   like mapleplot
%   \imaplesepline	  like \maplesepline, but ignored by the filter.
%
% ----------------------------------------------
% Implementation Details
% ----------------------------------------------
% The mapleinput, and maplettyout environments are similar to 
% \begin{verbatim}...\end{verbatim} but with several 
% important differences.
%
% - The spacing relative to the surrounding environment is different.
%
% - Page breaks are encouraged before commands, or after results,
%   and discouraged inbetween.
%
% - maplettyout and maplelatex environments are assumed to follow
%   mapleinput regions and so have less space above.  This allows us to
%   reduce the space between adjacent Maple regions without any
%   elaborate mechanism to detect when there have been intervening
%   paragraphs of text.
%
% - the size of the font for text regions is definable.  Use \MapleFont
%   to reset the font.
%
% - the  indentation of the environments can be indented by setting 
%   the value of \LeftMapleSkip  .
%
% - a prompt is automatically generated at the start of each line in
%   the case of the input environments.
%
% Much of the spacing and sizing information is parameterized.
% The following Macros control most of the spacing for the 
% Maple environments.  They are all resettable in the preamble of 
% your document. 
% 
% \AboveMapleSkip	- space above an environment
% \BelowMapleSkip	- space below an environment
% \AboveMaplePlot	- space above a Maple Plot 
% \BelowMaplePlot	- space below a Maple Plot
% \MaplePlotHeight	- vertical space reserved for a plot
% \MaplePlotWidth	- width reserved for a plot
% \MaplePlotAngle	- angle of rotatation
% \LeftMapleSkip 	- the amount of left indentation
% \MapleFont 		- The Maple font 
% \MapleSize 		- The size of the Maple font in mapleinput and 
%                          maplettyout
% \MapleLatexSize	- The size of the Maple fonts in maplelatex
% \MapleFirstLine	- controls ingoring first line feed
% \MaplePrompttrue 	- controls insertion of prompt char
% \MaplePromptString	- defines the prompt string
% \MaplePromptSecondary	- defines the secondary prompt string
% \MapleSkip		- amount of glue before and after
%			displayed text
% \MapleTab		- number of spaces per tab (8)
%
% Spacing, dimensions, etc.  
%
% These are all defined and given default values in the file
% mapleenv.def Most may be changed in your document preamble.
%
\input{mapleenv.def}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Define those Maple environments that are to be ignored by
% the Maple Filter.  
% 
% \begin{imapleinput} ...\end{imapleinput}
% \begin{imaplettyout} ...\end{imaplettyout}
% \begin{imaplelatex} ...\end{imaplelatex}
% \imaplesepline
% \imapleplot
%
% These environments are ignored by the Maple Filter.
%
% -- imapleinput
%
\def\imapleinput{
\removelastskip%
\MaplePrompttrue% prompt is required in this environment.
\if@minipage\removelastskip\vskip-1.3ex%
\else\vskip\AboveMapleSkip\fi%
\@SetupMapleTty{0}% The 0 indicates ignore first new line
\@BeginIMapleInput% 
}
%
\def\endimapleinput{%
  \@EndMapleTty%
  \removelastskip%
  \edef\@MapleIOType{\MapleIOType}
  \ifx\@MapleIOType\@MapleQuiet%
    \typeout{ .............Quiet Maple Command finished}
  \else
    \vskip\BelowMapleSkip% not usually followed by output...
  \fi%
  \@endpetrue
  \ignorespaces
}
%
% -- imaplettyout
%
\def\imaplettyout{
  \removelastskip%
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@BeginIMapleTtyout  % np indicates omit prompt
}
%
\def\endimaplettyout{%
  \@EndMapleTty%
  \removelastskip
  \vskip\BelowMapleSkip%
  \pagebreak[3]%
  \@endpetrue
  \ignorespaces
}%
%
% -- imaplelatex
%
%  an inert maple latex environment  (ignored by the filter)
%
\newenvironment{imaplelatex}%
{\vskip.5\AboveMapleSkip\vskip\z@\begin{maplelatex}}{\end{maplelatex}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define active mapleinput environments.
% 
% \begin{mapleinput} ...\end{mapleinput}
% \begin{maplettyout} ...\end{maplettyout}
% \begin{maplelatex} ...\end{maplelatex}
% 
% These parameterized environments are intended for reprocessing 
% by the Maple Filter.
%
% The [a] case is used by default.  
% The [q] is the quiet (suppressed)  mode.
% The [ni] (no input) behaves the same as [q]
% The [no] behaves the same as [a]
%
% Page breaks are inhibited immediately following the input
% environment.  This assumes that no extra space is 
% required below the region as it is followed by some
% form of Maple output region.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- mapleinput
%
\newlength\newleftskip%
\newbox\mapleinputbox%
\newenvironment{mapleinput}{%
%\def\@gobblefirst##1{\relax\egroup\par}
%\def\@gobblesecond##1##2{##1\egroup\par}
\def\@gobblesemicolons##1{##1}
\advance\hsize by -\LeftMapleSkip%
\global\setbox\mapleinputbox=\vbox\bgroup%
\everypar{\the\MaplePromptString\MaplePromptString=\MaplePromptSecondary\ }
\leftskip=\z@%
\parindent=\z@%
\parfillskip=0pt plus 1fil
\lineskiplimit=0\normalbaselineskip
\baselineskip=.85\normalbaselineskip
}{
\egroup% end of vbox
\par\removelastskip
\vskip\AboveMapleSkip%
\newleftskip=\leftskip%
\advance\newleftskip by \LeftMapleSkip%
\advance\newleftskip by \@totalleftmargin% needed for lists
\hbox{\hskip\newleftskip\box\mapleinputbox}
\vskip\BelowMapleSkip}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- maplettyout
%
\def\maplettyout{
  \removelastskip%
  \vskip 0pt plus 0pt minus 3pt%  
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@ifnextchar [{\@BeginMapleTtyout}{\@BeginMapleTtyout[a]}%
}
% 
\def\endmaplettyout{%
  \@EndMapleTty%
  \edef\@MapleIOType{\MapleIOType}
  \ifx\@MapleIOType\@MapleQuiet%
     \typeout{ .............Quiet Maple TTY finished}
  \else
    \vskip\BelowMapleSkip%
    \pagebreak[3]%
    \@endpetrue
    \ignorespaces
  \fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- maplelatex 
%
% This is essentially a wrapper around a display math environment
% It gobbles its content if the [q] or [no] options are in
% effect.
%
\newbox\maplebox
\def\maplelatex{\@ifnextchar [{\@maplelatex}{\@maplelatex[a]}}
%
\def\@maplelatex[#1]{%
\edef\@MapleIOType{#1}%
\gdef\MapleIOType{#1}%% for \ifx test%
\ifx\@MapleIOType\@MapleNoOutput%
\typeout{ .............Output Option [no]}%
\gdef\MapleIOType{q}%%  handle same as \@MapleQuiet  
\fi%
\global\setbox\maplebox=\vbox\bgroup%
\MakeSuperScript{^}%  Ensure these have normal interpretation
\MakeSubScript{_}%
}%
%
\def\endmaplelatex{\egroup%
\edef\@MapleIOType{\MapleIOType}%
\ifx\@MapleIOType\@MapleQuiet%   End the same as the verbatim's
\par%
%\@endpetrue
\else%
%\ifvmode\removelastskip\fi%
\nopagebreak[3]%
\centerline{%
\vbox{%
\hbox{\vrule height4pt depth0pt width 0pt}%
\unvbox\maplebox}}%
\vskip\BelowMapleSkip%
\everypar{}%
\par%

%\pagebreak[3]%
%\@endpetrue
%\ignorespaces
\fi%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- maplesepline
%
\newcommand{\maplesepline}{\vskip \parskip%
\hrule\@height\MapleSepLineHeight\@width\MapleSepLineWidth%
\vskip \parskip\relax}
%
% -- imaplesepline ( the inert form )
%
\let\imaplesepline\maplesepline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- \mapleIndent
%
% - Special Indentation Macro used to format procedures
%
\newdimen\Tab
\Tab=3ex
\def\mapleIndent#1{\hbox{\hskip#1\Tab\relax}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Special environments for in-line maple commands.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  \begin{maplegroup}				- maple exchange group
%  ...
%  ... and \mexpr{sin(x^2)} ...			- inline maple code
%  ...
%  \mapleinline{Inert}{TwoD}{int(sin(x^2),x);}{%	- for maple filter
%  {mapletex}{$\int{ .... }$}		        - for latex
%  ...
%  ...
%  \mapleresult					- location of inline results
%  \begin{maplelatex}				- actual displayed results
%  ...
%  \end{maplelatex}
%  \end{maplegroup}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% -- \mexpr 
%
% 	\mexpr{int(sin(x^2),x)} --- \mapleexpr{int(sin(x^2),x)}
%
% To make { and } visible in this verbatim environment, use \{ and \}
% Also, to make \ visible, use \\. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\mexpr{\setbox\@inlinebox=\hbox\bgroup\ttfamily\dosetup\let\\\BackSlash\@domexpr}
%
\def\mapleexpr{\bgroup\ttfamily\dosetup\let\\\BackSlash\@domexpr}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  \@dosetup	      sets up the character codes, etc. for verbatim
%  \@domexpr          completes the following inline math
%  \@gobblefirst      absorbs the inline math (not displaying it)
%  \@gobblesecond     absorbs the second following argument.
%  \@gobblesemicolons      absorbs semi-colons inside of the 1d mode.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dosetup{\let\do\@makeother\dospecials\postdospecials}
%
%\def\@domexpr#1{#1\egroup\fbox{\box\@inlinebox}}
\def\@domexpr#1{#1\egroup\box\@inlinebox}
%
\def\@gobblefirst#1{%
\relax\egroup%
% \fbox{\box\@inlinebox}%   %%% DEBUG %%%
\box\@inlinebox%
\setbox\@inlinebox=\hbox{}}
%
\def\@gobblesecond#1#2{%
#1\egroup\ignorespaces%
% \fbox{\box\@inlinebox}% %%% DEBUG %%%
\box\@inlinebox%
\setbox\@inlinebox=\hbox{}}
%
\def\@gobblesemicolons{\MakeActive{;}\@@gobblesemicolons}
%
{\MakeActive{;}\gdef\@@gobblesemicolons{\edef;{\relax}}}

%%% end of mexpr
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% -- \mapleinline
%
%	Essentially a four argument macro used to control the
%	display of inline material generated by Maple.
%
%	\mapleinline %
%	<status> 	% "active", or "inert"
%	<display mode>  % 1d or 2d
%	<verbatim source> % raw maple code as per \mexpr
%	<latex 2-D source> % latex representation
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \mapleinline{inert}{2d}{int(sin(x^2),x)}{ % used to generate display
% $\int{\sin(x^2),dx}$}	                    % updated by the filter
%
% Could use \@bsphack ... \@esphack for absorbing unwanted space not 
% currently used, but spacing inside this macro definition is 
% very important.
%
\edef\OneD{1d}\edef\TwoD{2d}% # tokens to identify modes
\newif\ifDisplay\Displayfalse
\newbox\@inlinebox\setbox\@inlinebox=\hbox{}%
\@ifundefined{@skiponetoken}{\gdef\@skiponetoken#1{\relax}}{\relax}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2-D output
% final output macro for mapleinline.
% include spacing above and below to ensure there is
% whitespace around the object when it occurs in
% a spreadsheet cell.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@doTwoD#1{\egroup%
%\@ifnextchar\cr{\@skiponetoken}{\relax}%
\@@doTwoD}%
%
\newdimen\cellwidth%
\def\@@doTwoD#1{%
\ignorespaces%
\setbox\@inlinebox=\hbox{#1}%
\ifMapleTableCell%  		  Used in maplespreadsheet
\cellwidth=\wd\@inlinebox%
\hbox{$\vcenter{\hsize=\cellwidth%
\hbox{\vrule height3pt depth0pt width 0pt}%
\box\@inlinebox%
\hbox{\vrule height0pt depth 3pt width 0pt}%  Actual output
}$}%
\egroup%
\else%				  Used inline ...
%\fbox{\hbox{\unhbox\@inlinebox}}\egroup% Actual output
\box\@inlinebox\egroup%
\fi%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1-D output
% Final output macro for mapleinline for 1-D output.
% The raw tokens must be dumped into the output stream so
% we use unhbox.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@doOneD#1{\MakeOther{\ } #1\egroup\unvbox\@inlinebox\relax\@mgobbleone}
\def\@mgobbleone#1{\relax\egroup}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mapleinline#1#2{%
% ignore first argument (inert or active)		
\def\[{$}\def\]{$}%		% needed for math mode.
\edef\DisplayType{#2}%		% 1d or 2d
\ifx\DisplayType\TwoD%
\let\Display\@doTwoD%	% display the 2-D representation
\global\Displaytrue%
\else%
\let\Display\@doOneD%	% display the 1-D representation
\global\Displayfalse%
\fi%
\bgroup%
\global\setbox\@inlinebox=\vbox\bgroup%
\obeylines%
\everypar{\the\MaplePromptString\MaplePromptString=\MaplePromptSecondary\ }
\ttfamily\dosetup\obeyspaces\let\\\BackSlash\Display%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% -- \begin{maplegroup} ... \end{maplegroup}
% -- \mapleresult
%
%	A environment used to group commands and result together into
%	one unit.  Inside, these are separated by \mapleresult.
%	The maple filter automatically deletes the part of a maplegroup
%	which follows \mapleresult and replaces it with new results.
%	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{maplegroup}{}{}
\def\maplegroup{\relax}
\def\endmaplegroup{\relax}
\let\mapleresult\relax   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Various Plot Configurations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Maple Plot Environemnts}
% 
% -- noplots  -- No Driver Available ?
%
\def\mapleplotname#1{
	\typeout{ ...using Plot file #1}%
	\vskip.5\MaplePlotHeight
        \centerline{\Large \bfseries Plot:  #1}
        \vskip.5\MaplePlotHeight
}
%
% -- epsfig.sty (used by dvips, etc)
%
\def\epsfigmapleplot#1{
	\parindent=0ex%
	\MaplePlotWidth  = 0.900\textwidth%
	\MaplePlotHeight = 0.651\textwidth%
	\MaplePlotHeight@Fudge=0.90\MaplePlotHeight%
	\MaplePlotWidth@Fudge =0.90\MaplePlotWidth%
	\ifvmode \removelastskip \else \par \parindent=0ex\removelastskip\fi
	%% \par
        \vskip \AboveMaplePlot
	%
	%  Plot sizes must be fudged because Maple .eps plots
	%  generated using Maple's built-in PostScript plot driver
	%  are 6.5 x 9 inches landscape, but included in portrait
	%  mode to a much smaller scale.
	%
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \relax
		    {}\hskip \LeftMapleSkip
		    \epsfig{figure=#1,%
			height=\MaplePlotHeight@Fudge,% scale before rotation
			width=\MaplePlotWidth@Fudge,%
			angle=\MaplePlotAngle}%
		}% end of hbox
	}% 
	{%
		\typeout{ ...Missing Plot File  #1}
		\noindent	% So \mapleplot can be used inside of
				% the LaTeX center environment.
		\vbox{\mapleplotname{#1} }%
	}%
	\par\removelastskip
        \vskip\BelowMaplePlot
	% \vskip-2\BelowMaplePlot{\relax}
	%%% \vspace*{-.3\MaplePlotHeight} 
	% \relax\noindent\ignorespaces
}% end of epsfigmapleplot def

%%
%Driver used exclusively by plots in Maple 11. The dimensions of the 
%plot are specified as point sizes in the 2nd and 3rd parameters.
%This driver is virtually the same as epsfigmapleplot, but without the rotation
%and the dimension fudge. 
%%
\def\maplepsplot#1#2#3{
	\parindent=0ex%
	\MaplePlotWidth  = #2%
	\MaplePlotHeight = #3%
	\ifvmode \removelastskip \else \par \parindent=0ex\removelastskip\fi
        \vskip \AboveMaplePlot
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \relax
		    {}\hskip \LeftMapleSkip
		    \epsfig{
		    	figure=#1,%
			height=\MaplePlotHeight,
			width=\MaplePlotWidth
		    }%
		}% end of hbox
	}% 
	{%
		\typeout{ ...Missing Plot File  #1}
		\noindent	% So \mapleplot can be used inside of
				% the LaTeX center environment.
		\vbox{\mapleplotname{#1} }%
	}%
	\par\removelastskip
        \vskip\BelowMaplePlot
}% end of maplepsplot def

%
% -- Oztex postscript driver
%
% Rotation is not supported.  so use Maple's commands to rotate.
% This can be done using the Maple command 
%
%	interface(plotoptions=`portrait,height=200,width=300`); 
%
% This is the same as mapleespfig, but with no rotation expected.
%
\def\oztexmapleplot#1{
	\ifvmode \removelastskip \else \par \fi
	\vskip \AboveMaplePlot
	%
	%  Plot sizes must be fudged because Maple .eps plots
	%  generated using Maple's built-in PostScript plot driver
	%  are 7.5 x 10 inches, but include an additional 0.5 inch
	%  white border within the PostScript BoundingBox.
	%
	\MaplePlotHeight@Fudge=1.133333\MaplePlotHeight
	\MaplePlotWidth@Fudge =1.100000\MaplePlotWidth
	\vskip -0.066667\MaplePlotHeight		%Fudge
	\noindent	% So \mapleplot can be used inside of
			% the LaTeX center environment.
	\IfFileExists{#1}{%
		\typeout{ ...including Plot #1 at size
		\the\MaplePlotWidth\space by \the\MaplePlotHeight}%
		\hbox{%
		    \hskip -0.05\MaplePlotWidth		%Fudge
		    \epsfig{figure=#1,%
			height=\MaplePlotWidth@Fudge,% scale before rotation
			width=\MaplePlotHeight@Fudge}%
%%oztex%% 			angle=\MaplePlotAngle}%
		    \hskip -0.05\MaplePlotWidth		%Fudge
		}%
	}% end of first case
	{% second case 
	    %\typeout{ ...Missing Plot File  #1}
	    { %
		\vskip.5\MaplePlotHeight%
		\centerline{\Large \bfseries Plot File = #1}
		\vskip.5\MaplePlotHeight %
		}% end of vbox
	}% end of second case
	\par
	\vskip -0.066667\MaplePlotHeight		%Fudge
	\vskip\BelowMaplePlot
	\vskip -\parskip\noindent\ignorespaces
} % end of oztexmapleplot

%%%%%%%%%%%%%%%%%%%%%%%%%
% Install the Driver.
%%%%%%%%%%%%%%%%%%%%%%%%%
\@ifundefined{Driver}{%
      \ifnoplots
	     \let\mapleplot\mapleplotname
	     \let\imapleplot\mapleplot
      \else
      \IfFileExists{epsfig.sty}{% Default to dvips
             \typeout{ ...Defaults to "dvips" Driver }
             \usepackage[dvips]{epsfig}
             \let\mapleplot\epsfigmapleplot
             \let\imapleplot\mapleplot
             \edef\Driver{dvips}}{%  no driver 
	     % generate vertical space containing file name
	     \let\mapleplot\mapleplotname
	     \let\imapleplot\mapleplot
	}
      \fi
}{\usepackage[\Driver]{epsfig}}
%
\def\maplesmartplot#1#2{\mapleplotname{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Maple Paragraph Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{Defining Automatic Style Generation Macros}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%--  Maple Worksheet Default Paragraph and Character Styles definitions
%
%   Unnamed Character styles are set up as {\textbf ... } while
%   named character styles are set up as macro calls of the form
%
%             \QTR{Style Name}{ ... data ... }
%
%   Paragraph styles are tagged by environments as in
%
%   \begin{flushleft} ... \end{flushleft}
%
%   This tagging also occurs for the user defined styles.
%
%   A list of style names actually used in a particular worksheet is
%   specified at the top of a Maple worksheet by macros of the form
%
%   \DefineCharStyle{... style name ...}
%   \DefineParaStyle{... style name ...}
%
%   If a macro by that name is already defined, then that definition
%   is used. Otherwise, a new macro is defined and set to the
%   document default style.
%
%   All style definitions, user defined, or system defined in this
%   style file, can be overridden in the document preamble simply
%   by providing a definition prior to The \Define...Style{...}
%   call.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%--------------------------------------------------------------------
% - Routine for Automatically defining Undefined Character Styles
%--------------------------------------------------------------------
\newif\if@def\@deffalse
\def\DefineCharStyle#1{
  \@ifundefined{#1}{\@deftrue}{\@deffalse}
  \if@def
    \typeout{Defining a new character style: #1}
    \expandafter\def\csname #1\endcsname##1{\relax {##1}}
  \fi}
%
%--------------------------------------------------------------------
% - Routine for Handling Undefined Paragraph Styles  
%
% These are handled as environments.  Blank spaces are allowed in 
% the environment names.
%--------------------------------------------------------------------
\def\DefineParaStyle#1{
\@ifundefined{#1}{\@deftrue}{\@deffalse}
\if@def
  \typeout{Defining new paragraph style: #1}
  \expandafter\newcommand \csname #1\endcsname[0]{\relax}%
  \expandafter\long\expandafter\def\csname end#1\endcsname{\relax}
\fi
}

%--------------------------------------------------------------------
% - Routine for Handling Undefined Character Styles
%
% This macro allows for macro names having spaces in them.
% Usage:
%
%     \QTR{macro name}{argument 1}
%
%--------------------------------------------------------------------
\@ifundefined{QTR}{%	
  \gdef\QTR#1#2{{\csname#1\endcsname{#2}}}}{\relax} % 
\@ifundefined{TEXTsymbol}{%
  \gdef\TEXTsymbol#1{\mbox{$#1$}}}{\relax}%

%--------------------------------------------------------------------
% - The Known (Pre-defined!) Maple Paragraph Styles
%---------------------------------------------------------------------
% \newenvironment{maplegroup}{}{}
\newenvironment{Maple Author}{\begin{center}\large\itshape\mdseries}{\end{center}}
\newenvironment{Maple subtitle}{\begin{center}\normalsize\upshape\mdseries}{\end{center}}
\newenvironment{Maple Bullet Item}{%
\renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}\item\null}{\end{itemize}}
\newenvironment{Maple Dash Item}{%
\begin{itemize}\item\null}{\end{itemize}}
\newenvironment{Maple Diagnostic}{\bfseries}{}
\newenvironment{Maple Error}{\bfseries}{}
%
\newenvironment{Maple Heading 1}[2][\section]
{#1{\Large\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 2}[2][\subsection]
{#1{\large\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 3}[2][\subsubsection]
{#1{\normalsize\bfseries\upshape {#2}}}
{}
\newenvironment{Maple Heading 4}[2][\subsubsection]
{#1{\normalsize\bfseries\itshape {#2}}}
{}
%
\newenvironment{Maple Normal}{\normalsize\rmfamily\mdseries}{}
\newenvironment{Maple Text Output}{\normalsize\ttfamily\mdseries}{}
\newenvironment{Maple Title}{\begin{center}\rmfamily\LARGE\upshape\ignorespaces}%
{\end{center}}
\newenvironment{Maple Warning}{\ttfamily}{}
%--------------------------------------------------------------------
% -- Fixed Width Environment is like a verbatim Version
%--------------------------------------------------------------------
%
\newbox\maplettybox%
\setbox\maplettybox=\hbox{}
%
\expandafter\def\csname MapleFixedWidth\endcsname{
  \removelastskip%
  \nopagebreak[3]% 
  \MaplePromptfalse	  % No prompt is required in this environment.
  \@SetupMapleTty{1}   % The 1 indicates "respect first new line"
  \@BeginMapleFixedWidth  % np indicates omit prompt
}
%
\expandafter\def\csname endMapleFixedWidth\endcsname{%
  \@EndMapleTty%
  \removelastskip
  \vskip\BelowMapleSkip%
  \pagebreak[3]%
  \@endpetrue
  \ignorespaces
}%
%
%------------------------------------------------------------------------------
% -- Regular Known Character styles
%
%        If spaces occur in name then define using \expandafter
%        as seen below, and invoke as QTR{name}{options}
%	 Otherwise, define and use as normal (i.e., using \def)
%
%------------------------------------------------------------------------------
\expandafter\def\csname Maple 2D Comment\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Input\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Math\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple 2D Output\endcsname#1{{\rmfamily\upshape #1}}
\expandafter\def\csname Maple Help Heading\endcsname#1{{\large\bfseries\sffamily\upshape #1}}
\expandafter\def\csname Maple Help Normal\endcsname#1{{\rmfamily\itshape #1}}
\expandafter\def\csname Maple 2D Comment\endcsname#1{{\rmfamily\itshape #1}}
\expandafter\def\csname Maple Maple Input\endcsname#1{{\ttfamily\upshape #1}}
\expandafter\def\csname Maple Output Labels\endcsname#1{{\ttfamily\upshape #1}}
\expandafter\def\csname Maple Plot Title\endcsname#1{{\large\sffamily\upshape #1}}
\expandafter\def\csname Maple Plot Text\endcsname#1{{\sffamily\upshape #1}}
\expandafter\def\csname Maple Popup\endcsname#1{{\bfseries\sffamily\upshape #1}}
\expandafter\def\csname Maple Hyperlink\endcsname#1{{\bfseries\rmfamily\itshape #1}}
%--------------------------------------------------------------------
% Hyperlink support (printing characteristics only)
%--------------------------------------------------------------------
\def\labelLink#1#2{\Hyperlink{#2}}
\def\docLink#1#2{\Hyperlink{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Maple Table Support
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{Defining Maple Spreadsheet Environments}
\typeout{Maple Spreadsheet and Table Support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Maple Spreadsheets and Tables Package
%%%
%%%  Maple displays its spreadsheets as a tabular arrays of cells.
%%%
%%% This is essentially a tabular environment
%%% with some pre and post processing. 
%%% The format is:
%%% \begin{maplespreadsheet}[spreadsheet01.tab]{|c|c|}
%%% \hline
%%% entry 1 &
%%% entry 2 &
%%% \mapleinline{inert}{2d}{1;}{xx} \\
%%% \hline
%%% entry 2,21 &
%%% entry 2,3  &
%%% \mapleinline{{1;} \\
%%% \hline
%%%\end{maplespreadsheet}
%%%
%%%  The cells are in typeset in text mode. The mathematics is
%%%  usually provided in \mapleinline in order to provide both the
%%%  Maple and the LaTeX encoding of the expression.
%%%
%%%  Maple's \multiline macro is used in the latex portion
%%%  of the \mapleinline macro in order to effect line wrapping.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifMapleTableCell%  % used to change vertical offset of a
			  % mapleinline inside table
\newdimen\multilinesep%
\multilinesep=1ex%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% maplespreadsheet - tabular environment whose entries are encoded
%%%	using mapleinline.
%%%
%%%	\begin{maplespreadsheet}[filename]{format}
%%%	...
%%%	\end{maplespreadsheet}
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maplespreadsheet{%
\@ifnextchar [{\@maplespreadsheet}{\@maplespreadsheet[]}
}
\def\@maplespreadsheet[#1]#2{%
\par\MapleTableCelltrue\begin{center}\begin{tabular}{#2}}%
\def\endmaplespreadsheet{%
\end{tabular}%
\end{center}%
\MapleTableCellfalse%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% maplemultiline - Used for stacking lines of maple input and output
%%%
%%% An implementation of mapleinline based on vbox and hbox.
%%% The tokens are parsed and dropped into hboxes which are in turn
%%% collected into a vbox.
%%%
%%% Each line of the multiline is followed by some extra space
%%% No extra space is required at the top as the multiline is
%%% used inside of \mapleinline, which provide's its own space
%%%
%%% \maplemultiline{x^2 + y^2\\(x - y)^{100}\\}
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tokens and utilities used by \maplemultiinline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\@linebuffer\setbox\@linebuffer=\vbox{\relax}
\newbox\@currentline\setbox\@currentline=\hbox{\relax}
\newdimen\@linebufferwidth  %%% DEBUG %%%
\newtoks\EndMultiLine%
\@ifundefined{@skiponetoken}{\gdef\@skiponetoken#1{\relax}}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \maplemultiline -
%%% for use primarily inside of table cells.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maplemultiline#1{%
{\def\\{\relax}%
\processcell#1\noexpand\\\EndMultiLine%
}%
%%% \@linebufferwidth=\wd\@linebuffer%%% DEBUG %%%
%\fbox{\@dumplinebuffer}%         %%% DEBUG %%%
\@dumplinebuffer%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processcell -
%%% start processing the contents of the cell
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processcell{\futurelet\@nexttoken\processline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processline
%%% - invokes \processfullline unless at the
%%% end of the cell. (skips over \cr's to
%%% avoid spacing problems)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processline{%
\ifx\@nexttoken\EndMultiLine%
\let\next\@skiponetoken%  % at end of cell.
\else%
\let\next\processfullline%% grab next line 
\fi%
% \cr's cause spacing problems.
\ifx\@nexttoken\cr\@skiponetoken\let\next\processline\fi%
\next%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \processfullline -
%%% - Adds currentline (as identified by \\)
%%% to the vbox \@linebuffer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\processfullline #1\\{%
\global\setbox\@currentline=\hbox{$#1$}
\@extendlinebuffer{\@currentline}%
\processcell}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \@extendlinebuffer - a stack of lines
%%% add currentline to end of \@linebuffer
%%%
%%% #1 is assumed to be a box. (hbox) and
%%% is reset at the end.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@extendlinebuffer#1{%
\ifvoid#1\else% 	% skip over blank lines
\ifvoid\@linebuffer%	% first line ?
\global\setbox\@linebuffer=\vtop{\copy#1}%
\else%			% add new lines
\global\setbox\@linebuffer=\vtop{%
\unvcopy\@linebuffer%
\copy#1%
\vskip\multilinesep%
}%
\fi%
\fi%
\global\setbox#1=\hbox{}% reset currentline
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \@dumplinebuffer -
%%% place @linebuffer on the output stream as
%%% a vbox.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@dumplinebuffer{%
\setbox\@linebuffer=\vtop{%
\hbox{\vrule height3pt depth0pt width 0pt}%
\unvbox\@linebuffer%
\unskip}%  
\box\@linebuffer%  A verticle box ...
\global\setbox\@linebuffer=\vbox{}%
\relax}

\newcommand{\Mapleoversetsp}[2]%
  {\mathop{\kern\z@#2}\limits^{\!\!\!#1}}
\newcommand{\Mapleundersetsp}[2]%
  {\mathop{\kern\z@#2}\limits_{\!\!\!#1}}

\newcommand{\Mapleoverset}[2]%
  {\mathop{\kern\z@#2}\limits^{#1}}
\newcommand{\Mapleunderset}[2]%
  {\mathop{\kern\z@#2}\limits_{#1}}

\endinput 
%%%% The End %%%%%
%%% </PRE>
